Study of quark and gluon jet identification in photoproduction at EIC

This paper presents a systematic study of the substructure of dijets produced in direct and resolved photoproduction events and subsequent quark and gluon jet identification in dijets, considering the kinematic reach of the upcoming Electron-Ion Collider (EIC) experiment. We investigate the substructure of jets produced in dijet photoproduction events with center-of-mass energies $\sqrt{s} = 64 \text{--}140$ GeV at the EIC.~Events are simulated using event generator PYTHIA and contributions from direct and resolved photoproduction subprocesses are analyzed at different energies.~Jets are reconstructed using longitudinally invariant $k_T$ algorithm within the FastJet framework.~Substructure of quark and gluon initiated jets in the selected dijet photoproduction sample is studied in detail by using jet-shape variables.~Predictions for subjet multiplicities and integrated jet shapes are presented in the gluon-initiated and quark-initiated jets in the dijet photoproduction events at the EIC energies.~These results demonstrate the feasibility of distinguishing quark and gluon jets in the photoproduction events at the EIC and provide a baseline for further QCD studies.

==> usepackages.tex <==
% === Core formatting ===
\usepackage[english]{babel}
\usepackage{graphicx}
\usepackage{dcolumn}
\usepackage{bm}
\usepackage{ragged2e}
\usepackage{enumitem}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{array}
\usepackage{tabularx}
\newcolumntype{Y}{>{\centering\arraybackslash}X}

% === Figures ===
%\usepackage[compatibility=false]{subcaption}
\usepackage{placeins}
\usepackage{adjustbox}

% === Editing tools (remove before submission) ===
\usepackage{comment}
\usepackage[normalem]{ulem}
% \usepackage{lineno}

% === Bibliography style ===
\bibliographystyle{apsrev4-2}

% === Must be near last ===
\usepackage[hidelinks,colorlinks=true,linkcolor=blue,citecolor=blue,urlcolor=blue]{hyperref}
\usepackage{bookmark}
\usepackage{cleveref}

% === Custom commands ===
\makeatletter
\newcommand*{\rom}[1]{\expandafter\@slowromancap\romannumeral #1@}
\makeatother
\renewcommand{\topfraction}{0.9}
\renewcommand{\bottomfraction}{0.9}
\renewcommand{\textfraction}{0.05}
\renewcommand{\floatpagefraction}{0.8}
